RocketQAv2: A Joint Training Method for Dense Passage Retrieval and Passage Re-ranking

In various natural language processing tasks, passage retrieval and passage re-ranking are two key procedures in finding and ranking relevant information. Since both the two procedures contribute to the final performance, it is important to jointly optimize them in order to achieve mutual improvement. In this paper, we propose a novel joint training approach for dense passage retrieval and passage re-ranking. A major contribution is that we introduce the dynamic listwise distillation, where we design a unified listwise training approach for both the retriever and the re-ranker. During the dynamic distillation, the retriever and the re-ranker can be adaptively improved according to each other's relevance information. We also propose a hybrid data augmentation strategy to construct diverse training instances for listwise training approach. Extensive experiments show the effectiveness of our approach on both MSMARCO and Natural Questions datasets. Our code is available at https://github.com/PaddlePaddle/RocketQA.

==> subfile/intro_old.tex <==
\section{Introduction}
\label{section:intro}
In recent years, dense passage retrieval has become an important information seeking approach in identifying relevant contents~\citep{dpr2020}. The underlying idea is to represent both queries and passages as low-dimensional vectors, so that the relevance can be measured via vector similarity. More recently, it has been found that a subsequent procedure of \emph{passage re-ranking} can further improve the retrieval quality of initial passage retrieval results. Such a retrieval refinement procedure is particularly useful in a variety of natural language processing tasks, including question answering~\citep{mao2021reader,multihopqa}, dialogue system~\citep{conversation,henderson2017efficient} and entity linking~\citep{entitylinking,wu2019scalable}. 


%Passage retrieval and passage re-ranking are both important techniques in information retrieval.  Passage retrieval aims to quickly find relevant information from a large set of knowledge. More recently, dense passage retrieval has become the mainstream method for passage retrieval, which indexes all the passages in a low-dimensional and continuous space~\citep{dpr2020}. Passage re-ranking aims to refine the initial retrieval results in passage retrieval. It has been shown that dense passage retrieval and passage re-ranking are widely used to improve the variety of natural language processing tasks, including question answering~\citep{mao2021reader,multihopqa}, dialogue system~\citep{conversation,henderson2017efficient} and entity linking~\citep{entitylinking,wu2019scalable}. 

Typically, the retriever in dense passage retrieval and the re-ranker in passage re-ranking are implemented separately, which are naturally correlative following a \emph{retrieve-then-rerank} pipeline. Considering the isolation of the two modules in retrieval and re-ranking, several studies try to enhance the connection between them in order to achieve mutual improvement~\citep{rocketqa, metzler2021rethinking, Huang2020embedding}. 
On one hand, the retriever needs to capture the relevance knowledge from the re-ranker, since the re-ranker usually adopts a more complicated yet powerful architecture~\citep{rocketqa,google2020augmentation}. On the other hand, the re-ranker should be specially optimized according to the preceding results of the retriever, since it is built on top of the retriever, otherwise it will result in a sub-optimal performance~\citep{Huang2020embedding,Gao2020ModularizedTR}.
However, the existing methods are limited by the iterative training of two modules, which makes the training process more complicated. A basic idea is that the two modules could be jointly optimized, so that their information can be transferred and utilized from each other. 


\ignore{
Typically, the retriever in dense passage retrieval and the re-ranker in passage re-ranking are implemented separately, following a \emph{retrieve-then-rerank} pipeline. Considering the isolation of the two procedures in retrieval and re-ranking, several studies try to enhance the connection between them in order to achieve mutual improvement~\citep{rocketqa,metzler2021rethinking,Huang2020embedding}.
A basic idea is that the two modules should be jointly optimized, so that their information can be transferred and utilized in each other. On one hand, the retriever needs to capture the relevance knowledge from the re-ranker, since the re-ranker usually adopts a more complicated yet powerful architecture~\citep{rocketqa,google2020augmentation}. 
On the other hand, the re-ranker should be specially optimized according to the preceding results of the retriever, since it is  built on top of the retriever, otherwise it will result in a sub-optimal performance~\citep{Huang2020embedding,Gao2020ModularizedTR}.
}

%Although performance improvement can be achieved by heuristically connecting the retriever and the re-ranker, it is  challenging to implement a joint optimization approach for effectively integrating the two modules. 
Several existing studies attempted joint training of retriever and reader~\cite{REALM, sachan2021end, dpr2020}, but no study tried joint training of these two closely related modules. A fundamental issue is that both modules are usually optimized in different ways, so that the relevance assessment information (\eg the relevance distributions over candidates) of one module over the candidate passages is hard to be referred to or utilized in the other module. Specially, the retriever is usually trained by sampling a number of in-batch negatives to maximize the probabilities of relevant passages and minimize the probabilities of the sampled negatives~\citep{MEBERT,dpr2020}, where the relevance assessment is learned considering the entire list of relevant passages and negatives (called \emph{listwise} optimization\footnote{Note that instead of focusing on the full ranking of candidates as in learning to rank~\citep{cao2007learntorank}, we use ``listwise'' to indicate that the relevance assessment is made based on the entire list of candiates.}). As a comparison, the re-ranker is usually implemented in a pointwise or pairwise manner~\citep{nogueira2019passage,rocketqa,wang2019multi}, where the relevance assessment is learned based on a single passage or a pair of passages. 
Therefore, the learned relevance assessment from the two modules are characterized in different ways, which prevents direct information interaction between them and brings obstacles to joint training. 

%Therefore, it is important to derive a unified optimization form in order to share relevance assessment information across the two modules. In particular, both modules adopt 

%has been achieved by considering the dependency of the retriever and the re-ranker, however, there are problems in these methods: Limited to the form of individual training, the process of mutually fitting result distribution increases the training cost, the result distributions of the retriever and the re-ranker also cannot be fitted well with individual training.To address these problems, we propose to jointly train the retriever and the re-ranker in a unified architecture. During joint training, both two models are able to directly interact to each other by a unified training process. While the training cost will also decrease because there is no need to iteratively train the two models.



\ignore{Typically, the retriever in dense passage retrieval and the re-ranker in passage re-ranking are trained individually. In view of the natural characteristic of the retrieve-then-rerank pipeline, existing studies~\citep{rocketqa,metzler2021rethinking,Huang2020embedding} show that considering the dependency of the retriever and the re-ranker brings improvement for both two models.
Specifically, to improve the performance, the retriever needs to learn the knowledge of the re-ranker since the re-ranker usually has better ranking capabilities~\citep{rocketqa,google2020augmentation}. While the re-ranker should be re-optimized according to the preceding retriever's result distribution, since the current re-ranker are designed for existing retrieval scenarios, otherwise it will result in a sub-optimal performance~\citep{Huang2020embedding,Gao2020ModularizedTR}.
Although improvement has been achieved by considering the dependency of the retriever and the re-ranker, however, there are problems in these methods: Limited to the form of individual training, the process of mutually fitting result distribution increases the training cost, the result distributions of the retriever and the re-ranker also cannot be fitted well with individual training.
To address these problems, we propose to jointly train the retriever and the re-ranker in a unified architecture. During joint training, both two models are able to directly interact to each other by a unified training process. While the training cost will also decrease because there is no need to iteratively train the two models.
}

\ignore{Although the idea is appealing, it is not easy to implement it due to two major issues:
(1) How to design the approach of joint training? In order to achieve information interaction of the retriever and the re-ranker and make the result distributions of two models fit to each other, a proper joint training approach is required. (2) How to design the sampling approach in joint training? The original sampling methods of the retriever and the re-ranker are not suitable for the joint training method. Existing sampling approach of the retriever use in-batch negative sampling~\cite{MEBERT,dpr2020,rocketqa}, which brings a large number of weak negatives in training, and the re-ranker usually applies a point-wise or pair-wise manner~\citep{nogueira2019passage,rocketqa,wang2019multi}, which do not leveraging much negatives. Thus a suitable and unified sampling method needs to be designed. 
By leveraging the dual-encoder based retriever and the cross-encoder based re-ranker architecture, we focus on developing the right training scheme of jointly training the retriever and the re-ranker.
}
%The dual-encoder based retriever and the cross-encoder based re-ranker have different training forms. Specifically, the retriever usually trained in an in-batch manner with cross-entropy, which collect a large number of instances in the same batch as easy negatives. While the re-ranker usually trained in a point-wise or a pair-wise form with a few negatives. This difference brings the challenge for the implement of joint training. It is necessary to design a suitable training approach that can accommodate to both models for fitting the two result distributions.

\ignore{
In light of these challenges, we first propose the dynamic soft distillation as the joint training approach of the retriever and the re-ranker. We optimize the result distributions of the retriever and the re-ranker by the minimize the KL-divergence of the scores of the candidate instances. Inspired by knowledge distillation~\citep{Hinton2015distilling}, we regard the re-ranker which is more powerful on ranking as the teacher model and regard the retriever as the student model. During joint training, we use the re-ranker to obtain the soft label to guide the retriever, and the re-ranker also makes efforts to fit the result distribution of the retriever. In this way, the distillation becomes a dynamic process, where the soft label is dynamic changing with model updating. This will bring a multi-view information of the instances, as discussed in Sec~\ref{section:discussion}.
Besides, we design a unified list-wise sampling method to sample instances for the joint training architecture. Prior works mainly using in-batch sampling to obtain a large set of weak negatives, which may not suit for distillation. Differently, we sample hard negative in a list-wise manner, where all the negatives for a query are hard negatives, guaranteeing the data quality of the distillation process.}


In order to address these issues, our idea is to unify the optimization form for both retriever and re-ranker, so that achieve information interaction across the two modules. Specially, we adopt the listwise training approach for both retriever and re-ranker, where the relevance assessment is made according to a list of positive and negative passages. In this way, given a list of candidates to evaluate, the relevance distributions from retriever and re-ranker can be referred to by each other. The retriever captures the interaction knowledge from the re-ranker, while the re-ranker is optimized to fit the relevance distribution of the retriever synchronously. 
To implement this optimization form, a key point is to design the sampling method for the construction of instance list, since it needs diverse relevance scores in a instance list to better simulate the relevance distribution. Existing methods often consider randomly sampled negatives (regarded as weak negatives) in training. But in our listwise optimization form, weak negatives with low relevance scores in both retriever and re-ranker may lead to limited information learned, which is demonstrated in our experiments. We further consider utilizing only hard negatives in instance list for better learning. 

To this end, we propose a novel joint optimization approach for dense passage retrieval and passage re-ranking~(called \textbf{RocketQAv2}). Considering the aforementioned issues, we have made two important technical contributions. 
First, we adopt a unified listwise form to train both retriever and re-ranker, so that their relevance assessment distributions can be shared by each other. We further design the dynamic distillation mechanism to couple the two modules. In this process, the retriever tries to approximate the relevance distribution of the re-ranker to enhance the retrieval quality. While, the re-ranker learns to adjust its parameters, so that the output will be better suited and optimized for the retriever. 
Second, we propose hybrid data augmentation that is adapted to the distillation process, which is the key support for dynamic distillation.
The two technical contributions make it possible to effectively jointly train the retriever and the re-ranker for improving dense passage retrieval and passage re-ranking. 

%design the dynamic soft distillation as the training approach of the retriever and the re-ranker to implement the joint learning, that enables both models to directly interact to each other and realizes the mutual fitting of the result distributions of both models. 


%Second, we propose the unified list-wise sampling method that be adapted to the distillation process and enables the model to make more hard negatives be exposed in joint training, which is an important support to the dynamic soft distillation. The improvements in the two aspects make it possible to effectively and efficiently jointly train the retriever and the re-ranker for improving dense passage retrieval and passage re-ranking. 

The contributions of this paper can be summarized as follows:
\begin{itemize}
    \item We propose a novel approach that jointly trains the retriever in dense passage retrieval and the re-ranker in passage re-ranking. It is the first time that joint training has been implemented for the two modules.
    \item We make two major technical contributions by introducing dynamic distillation and hybrid data augmentation to support the proposed joint learning architecture.
    \item Extensive experiments show that our approach significantly outperforms previous state-of-the-art models on both MSMARCO and Natural Questions datasets.
\end{itemize}

==> subfile/method_old.tex <==
\section{Methodology}
In this section, we describe a novel joint training method for dense passage retrieval and passage re-ranking~(called \textbf{RocketQAv2})

\subsection{Overview}
\label{section:overview}
In this work, we consider two tasks including dense passage retrieval and passage re-ranking, which are described as follows.

%Given a query $q$, the aim of dense passage retrieval is to retrieve $k$ most relevant passages from a large collection of $M$ text passages. The dual-encoder~(DE) architecture is widely adopted by prior works~\citep{dpr2020, MEBERT, rocketqa}, where two separate dense encoders $E_P(\cdot)$ and $E_Q(\cdot)$ are used to map any passage or query to a $d$-dimensional real-valued vector and build an index for all $M$ passages for retrieval. The similarity between the query $q$ and the passage $p$ is defined using the dot product:
Given a query $q$, the aim of \emph{dense passage retrieval} is to retrieve $k$ most relevant passages from a large collection of $M$ text passages. The dual-encoder~(DE) architecture is widely adopted by prior works~\citep{dpr2020, MEBERT, rocketqa}, where two separate dense encoders $E_P(\cdot)$ and $E_Q(\cdot)$ are used to map passages and queries to $d$-dimensional real-valued vectors (a.k.a., embeddings) separately, and then an index of all passage embeddings is built for efficient retrieval. The similarity between the query $q$ and the passage $p$ is defined using the dot product:
\begin{equation}
\label{equation:sim_definition}
s_\text{de}(q, p)=E_Q(q)^{\top} \cdot E_P(p).
\end{equation}
\ignore{
Let $p^+$ denotes positive passage and $p^-$ denotes negative passage, the above similarity are usually learned by optimizing the negative log likelihood of the positive passage:
\begin{equation}
\label{equation:L_Q}
\small
L = -\frac{1}{N} \sum_{\langle q, p+\rangle} \log \frac{e^{s_\text{de}(q, p^+)}}{e^{s_\text{de}(q, p^+)} + \sum_{p^-} e^{s_\text{de}(q, p^-)}}.
\end{equation}
Prior works often adopt in-batch negative sampling to obtain amount of in-batch negatives~(weak negatives) to boost the performance of dual-encoder~\citep{dpr2020,MEBERT}. 
}

Given a list of candidate passages retrieved by a passage retriever, the aim of \emph{passage re-ranking} is to further improve the retrieval results with a re-ranker, which estimates a relevance score $s(q,p)$ measuring the relevance level of a candidate passage $p$ to a query $q$. 
Among the implementations of the re-ranker, a PLM-based cross-encoder~(CE) usually achieves superior performance~\citep{nogueira2019passage, qiao2019understanding}, which can better capture the semantic interactions between the passage and the query, but requires more computational efforts than the dual-encoder. 
To compute the relevance score $s_\text{ce}(q,p)$, a special token \textsc{[SEP]} is inserted between $q$ and $p$, and then the representation at the \textsc{[CLS]} token from the cross-encoder is fed into a learned linear function. % (typically trained with a pointwise or pairwise objective). 



% Here, we propose the joint training architecture for dense passage retrieval and passage re-ranking. Figure~\ref{fig:pipeline} presents the overall architecture. Our approach consists of two major technical contributions, namely dynamic distillation and hybrid data augmentation. 
% Section~\ref{section:distill} describes dynamic distillation that couples the two modules by the relevance distribution, which is the core of the joint training architecture. Section~\ref{section:negative-sampling} describes hybrid data augmentation that enables the listwise optimization form to touch diverse instances, which provides the data support for joint training. Furthermore, we describe the learning details and deeper discussion in Section~\ref{section:discussion}.
Usually, the passage retriever and the passage re-ranker are learned separately, which cannot be trained in an end-to-end way due to inconsistent optimization objectives and lack of high-quality training instances.   
To address these issues, our approach introduces two two major technical contributions:
(1) dynamic distillation (Section~\ref{section:distill}) unifies the optimization objective for the retriever and re-ranker in a listwise form;  (2) hybrid data augmentation (Section~\ref{section:distill}) generates sufficient training instances for supporting the listwise optimization. Furthermore, we present the learning details and related discussion in Section~\ref{section:discussion}. 


\ignore{Previous studies trained the retriever and the re-ranker individually. However, both retriever and re-ranker are actually highly related and dependent, the score distributions from retriever and re-ranker need to be referred to by each other for optimal performance. Therefore, we propose the joint training architecture for dense passage retrieval and passage re-ranking, including two technical contributions: Dynamic distillation couples the two modules by the score distribution, hybrid data augmentation method enables the joint training architecture to touch hard negatives from different sampling approach as a guarantee for dynamic distillation. Figure~\ref{fig:model} presents the overall architecture. }

\begin{figure}
	\centering 
	\includegraphics[width=0.49\textwidth]{figure/model.pdf}
	\caption{The illustration of dynamic listwise distillation. }
	\label{fig:model} 
% \vspace{-3mm}
\end{figure}


% \subsection{Dynamic Distillation}
% \label{section:distill}

% % design a training approach that makes the information of the retriever and the re-ranker interact mutually, we propose the dynamic soft distillation approach as the cornerstone of our joint training architecture.

% To implement joint training of the retriever and the re-ranker, designing a unified and effective training approach is an important issue. As the preliminaries of dynamic distillation , we first introduce a unified listwise form for the training retriever and re-ranker.
% %Here, we propose a specific training approach designed for the joint training of both models, which aims to enable the information of both modules interact directly with joint training.

% % With the obtained $\mathcal{P}_q$ by the unified list-wise sampling, we can apply the dynamic soft distillation to jointly train the two models. 
% Given a query $q$ in a query set $\mathcal{Q}$ and the corresponding list of support passages $\mathcal{P}_q = \{p_{q,i}\}_{1 \leq i \leq m}$ related to query $q$, following the notations in Section~\ref{section:overview}, we obtain the relevant scores $S_\text{de}(q) = \{s_\text{de}(q, p)\}_{p\in \mathcal{P}_q}$ and $S_\text{ce}(q) = \{s_\text{ce}(q, p)\}_{p\in \mathcal{P}_q}$ of a query $q$ and passages in $\mathcal{P}_q$ from the dual-encoder-based retriever and the cross-encoder-based re-ranker, respectively. Thus, the relevance assessment is made according to a list of instances and the score distributions from retriever and re-ranker can be referred to by each other.

% Base on the preliminaries, the idea of dynamic distillation is to make the relevance  distribution of both modules can be shared with each other. Figure~\ref{fig:model} is a visual explanation. Different from RocketQA that conducts hard distillation approach through labeled data~\citep{rocketqa}, we adopt soft label to enable the score distribution of both models to interact mutually and also mitigate the under-learning of data with ambiguous scores. To achieve the mutual-adaption, we minimize the KL-divergence between the candidate scores $S_\text{de}(q)$ and $S_\text{ce}(q)$ after normalization:
% \begin{equation}
% \label{equation:kl_divergence}
% \mathcal{L}_{\text{KL}} = \sum_{q \in \mathcal{Q}, p \in \mathcal{P}_q}
% \tilde s_\text{de}(q, p) \cdot {\log \frac{\tilde s_\text{de}(q,p)}{\tilde s_\text{ce}(q, p)}},
% \end{equation}
% where
% \begin{equation}
% \label{equation:kl_divergence}
% \tilde s_\text{de}(q, p) = \frac{e^{s_\text{de}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{de}(q, p')}}
% \end{equation}
% and
% \begin{equation}
% \label{equation:kl_divergence}
% \tilde s_\text{ce}(q, p) = \frac{e^{s_\text{ce}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{ce}(q, p')}}.
% \end{equation}
% % where $p \in \mathcal{P}_q$. 

% Generally speaking, a re-ranker has better ranking performance than a retriever. Thus, during joint training, re-ranker acts more as a teacher, which determines the direction of KL-divergence. At the same time, the re-ranker is dynamically updated according to the relevance distribution of retriever at each training step, which is the origin of the name \emph{dynamic distillation}.

% In order to provide guidance for joint training, we also adopt a cross-entropy loss for cross-encoder based on passages in $\mathcal{P}_q$ with supervised information:
% \begin{equation}
% \label{equation:sup}
% \small
% \mathcal{L}_\text{sup} = -\frac{1}{N} \sum_{q \in \mathcal{Q}, p^+} \log \frac{e^{s_\text{ce}(q, p^+)}}{e^{s_\text{ce}(q, p^+)} + \sum_{p^-} e^{s_\text{ce}(q, p^-)}},
% \end{equation}
% where $p^+$ and $p^-$ denote the positive passage and negative passage in $\mathcal{P}_q$, respectively.

% We combine the KL-divergence loss and the supervised cross-entropy loss defined in Eq.(\ref{equation:kl_divergence}) and Eq.(\ref{equation:sup}) to obtain the final loss function:
% \begin{equation}
% \label{equation:tot_loss}
% \mathcal{L}_{\text{final}} = \mathcal{L}_{\text{KL}} + \mathcal{L}_{\text{sup}}.
% \end{equation}



% The dynamic distillation achieves the mutual improvement of both retriever and re-ranker with unified listwise form of joint training, where the retriever captures the interaction knowledge from the re-ranker, while the re-ranker is optimized synchronously to fit the score distribution of the retriever. 

\subsection{Dynamic Listwise Distillation}
\label{section:distill}

% design a training approach that makes the information of the retriever and the re-ranker interact mutually, we propose the dynamic soft distillation approach as the cornerstone of our joint training architecture.
Since the re-ranker adopts the more capable cross-encoder architecture,  it has become a common strategy to distill the re-ranker for learning the retriever.  %However, such a distillation process  
However, in prior studies~\cite{}, the retriever and re-ranker are usually optimized with different objectives, and the parameters of the re-ranker are \emph{frozen}, which cannot fully fuse the relevance information captured by the two components. 
Inspired by early works in learning to rank~\cite{}, we design a unified listwise optimization objective 
for training both the retriever and re-ranker, and also update the parameters of the re-ranker, so that the two components can adaptively improve each other. %We refer to such a distillation way as \emph{dynamic listwise distillation}.

%In prior studies~\cite{}, the re-ranker is first learned and then distilled to improve the retriever.   During the distillation, the parameters of the re-ranker are \emph{frozen},  A major obstacle of jointly training the retriever and re-ranker is that both components usually adopt different optimization objectives. Inspired by early works in learning to rank~\cite{}, we propose a unified listwise optimization objective  for training both the retriever and re-ranker.

%To implement joint training of the retriever and the re-ranker, designing a unified and effective training approach is an important issue. As the preliminaries of dynamic distillation , we first introduce a unified listwise form for the training retriever and re-ranker.
%Here, we propose a specific training approach designed for the joint training of both models, which aims to enable the information of both modules interact directly with joint training.

% With the obtained $\mathcal{P}_q$ by the unified list-wise sampling, we can apply the dynamic soft distillation to jointly train the two models. 

Given a query $q$ in a query set $\mathcal{Q}$ and the corresponding list of supporting passages $\mathcal{P}_q = \{p_{q,i}\}_{1 \leq i \leq m}$ related to query $q$, following the notations in Section~\ref{section:overview}, we can obtain the relevance scores $S_\text{de}(q) = \{s_\text{de}(q, p)\}_{p\in \mathcal{P}_q}$ and $S_\text{ce}(q) = \{s_\text{ce}(q, p)\}_{p\in \mathcal{P}_q}$ of a query $q$ and passages in $\mathcal{P}_q$ from the dual-encoder-based retriever and the cross-encoder-based re-ranker, respectively. %Here, we assume that the retriever and the re-ranker have been initially trained. 


The main idea is to first normalize the relevance scores into relevance distributions over the candidate list, and then adaptively reduce the  difference of the two distributions from the retriever and the ranker so as to mutually improve each other.   
 To achieve the mutual adaption in the distillation, we minimize the KL-divergence between the two relevance distributions $\{\tilde s_\text{de}(q, p)\}$ and $\{\tilde s_\text{ce}(q, p)\}$:
 % candidate scores $S_\text{de}(q)$ and $S_\text{ce}(q)$ after normalization:
\begin{equation}
\label{equation:kl_divergence}
\mathcal{L}_{\text{KL}} = \sum_{q \in \mathcal{Q}, p \in \mathcal{P}_q}
\tilde s_\text{de}(q, p) \cdot {\log \frac{\tilde s_\text{de}(q,p)}{\tilde s_\text{ce}(q, p)}},
\end{equation}
where the relevance scores are normalized below:
\begin{eqnarray}
\tilde s_\text{de}(q, p) &=& \frac{e^{s_\text{de}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{de}(q, p')}},\label{equation:kl_divergence}\\
%\end{equation}
%and
%\begin{equation}
%\label{equation:kl_divergence}
\tilde s_\text{ce}(q, p) &=& \frac{e^{s_\text{ce}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{ce}(q, p')}}\label{equation:kl_divergence}.
\end{eqnarray}



%is a visual explanation. Different from RocketQA that conducts hard distillation approach through labeled data~\citep{rocketqa}, we adopt soft label to enable the score distribution of both models to interact mutually and also mitigate the under-learning of data with ambiguous scores.

%We normalize the relevance scores into relevance distributions over the candidate list, and further reduce the  difference of the two distributions from the retriever and the ranker so as to mutually improve each other.   

%Thus, the relevance assessment is made according to a list of instances and the score distributions from retriever and re-ranker can be referred to by each other.

\ignore{
Base on the preliminaries, the idea of dynamic distillation is to make the relevance  distribution of both modules can be shared with each other. Figure~\ref{fig:model} is a visual explanation. Different from RocketQA that conducts hard distillation approach through labeled data~\citep{rocketqa}, we adopt soft label to enable the score distribution of both models to interact mutually and also mitigate the under-learning of data with ambiguous scores. To achieve the mutual-adaption, we minimize the KL-divergence between the candidate scores $S_\text{de}(q)$ and $S_\text{ce}(q)$ after normalization:
\begin{equation}
\label{equation:kl_divergence}
\mathcal{L}_{\text{KL}} = \sum_{q \in \mathcal{Q}, p \in \mathcal{P}_q}
\tilde s_\text{de}(q, p) \cdot {\log \frac{\tilde s_\text{de}(q,p)}{\tilde s_\text{ce}(q, p)}},
\end{equation}
where
\begin{equation}
\label{equation:kl_divergence}
\tilde s_\text{de}(q, p) = \frac{e^{s_\text{de}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{de}(q, p')}}
\end{equation}
and
\begin{equation}
\label{equation:kl_divergence}
\tilde s_\text{ce}(q, p) = \frac{e^{s_\text{ce}(q, p)}}{\sum_{p' \in \mathcal{P}_q} e^{s_\text{ce}(q, p')}}.
\end{equation}
% where $p \in \mathcal{P}_q$. 
}
%Generally speaking, a re-ranker has better ranking performance than a retriever. Thus, during joint training, re-ranker acts more as a teacher, which determines the direction of KL-divergence. At the same time, the re-ranker is dynamically updated according to the relevance distribution of retriever at each training step, which is the origin of the name \emph{dynamic distillation}.

In order to provide guidance for the joint training, we also adopt a cross-entropy loss for cross-encoder based on passages in $\mathcal{P}_q$ with supervised information:
\begin{equation}
\label{equation:sup}
\small
\mathcal{L}_\text{sup} = -\frac{1}{N} \sum_{q \in \mathcal{Q}, p^+} \log \frac{e^{s_\text{ce}(q, p^+)}}{e^{s_\text{ce}(q, p^+)} + \sum_{p^-} e^{s_\text{ce}(q, p^-)}},
\end{equation}
where $p^+$ and $p^-$ denote the positive passage and negative passage in $\mathcal{P}_q$, respectively.
We combine the KL-divergence loss and the supervised cross-entropy loss defined in Eq.(\ref{equation:kl_divergence}) and Eq.(\ref{equation:sup}) to obtain the final loss function:
\begin{equation}
\label{equation:tot_loss}
\mathcal{L}_{\text{final}} = \mathcal{L}_{\text{KL}} + \mathcal{L}_{\text{sup}}.
\end{equation}



Figure~\ref{fig:model} presents the illustration of the dynamic listwise distillation. The re-ranker will be first optimized with labeled lists, and then it produces relevance distributions to train the retriever.  
Such an optimization process can be naturally modeled by the asymmetric KL-divergence loss in Equation~\ref{equation:kl_divergence}.  Unlike RocketQA that conducts hard pseudo labeled data~\citep{rocketqa}, we utilize soft labels (\ie predicted relevance distributions) for relevance distillation. Besides, we dynamically update the parameters of the re-ranker in order to adaptively fuse the relevance information from both the retriever and the ranker.
To discriminate from the previous static distillation based on pseudo labels, we refer to our method as \emph{dynamic listwise distillation}.

\begin{figure}
	\centering 
	\includegraphics[width=0.49\textwidth]{figure/data.pdf}
	\caption{The detail of hybrid data augmentation.  }
	\label{fig:data} 
% \vspace{-3mm}
\end{figure}


\subsection{Hybrid Data Augmentation}
\label{section:negative-sampling}
% The implement of joint training is limited by the different sampling approaches of the retriever and the re-ranker~\citep{dpr2020, nogueira2019passage, rocketqa}. The traditional sampling methods of two models often use in-batch negative sampling or in a pointwise or a pairwise manner, which are not suitable for the proposed joint learning architecture. Concretely, in dynamic distillation, the adoption of corresponding list of support passages $\mathcal{P}_q$ requires a list of training instances that has diverse relevance assessment to simulate the relevance distribution. Here, we propose the hybrid data augmentation method for generating a list of high-quality instances to both retriever and re-ranker for supporting the dynamic distillation. 
To preform the dynamic listwise distillation, we first need to generate the support passage list $\mathcal{P}_q$ for query $q$. A traditional method is to use in-batch negative sampling~\citep{dpr2020, nogueira2019passage, rocketqa}. 
However, since we rely on the relevance distribution in the distillation, it is important to include representative passages  that cover different relevant cases for effective distillation. In other words, we should be able to generate  more diverse, high-quality  instances for constructing  the support passage list.

% Given a query $q$, the positive and negative passages $\mathcal{P}_q = \{p_{q,i}\}_{1 \leq i \leq m}$ is sampled in a listwise manner, which matches the form of listwise training architecture in Eq.(\ref{equation:tot_loss}).


As shown in Figure~\ref{fig:data}, the hybrid data augmentation includes undenoised instance and denoised instance. First, we utilize RocketQA retriever to retrieve top-$n$ passages from the corpus. For undenoised instance, we randomly sample the undenoised hard negative and regard positive with label as positive based on retrieved passages. For denoised instance, we utilize RocketQA re-ranker to denoise the retrieved passage that remove the passages that are predicted as negatives by the cross-encoder with low confidence scores. We also obtain denoised positive that predicted as positive by the cross-encoder with high confidence scores for denoised instance. For each instance list in undenoised instance of denoised instance, we use one positive and rest of instances are hard negatives.

\ignore{
The first type of instances including labeled passages as positives and a random subset of recalled passages by the existing retriever as hard negatives. Concretely, we use the step-$1$ dual-encoder in RocketQA~\cite{rocketqa} to recall amount of related passages~(\eg top-1000) of query $q$. We randomly sample $n$ passages from recalled passages as hard negatives.
Moreover, since top-retrieved passages that are likely to be false negatives, we use the denoised hard negatives and positives as the second type of instances similar to prior work~\citep{rocketqa}. We utilize the step-$1$ cross-encoder to filter positives and hard negatives, note that this part of positives are not leveraged in RocketQA. Finally, we use one positive passage and $n$ hard negative passages in the sampled passage list $\mathcal{P}_q$ of the query $q$.
}

Compared with prior studies, our hybrid data augmentation method improves the relevance diversity of instances list $\mathcal{P}_q$. $\mathcal{P}_q$ with full of hard negatives can better simulate the relevance distributions of both retriever and re-ranker, which benefits the dynamic distillation process. On the contrary, weak negatives in $\mathcal{P}_q$ are easily learned with low relevance scores, while dynamic distillation process actually needs more hard negatives that have ambiguous scores and contain more under-learning information.



\begin{figure}
	\centering 
	\includegraphics[width=0.48\textwidth]{figure/pipeline.pdf}
	\caption{The overall joint training architecture of RocketQAv2.}
	\label{fig:pipeline} 
% \vspace{-3mm}
\end{figure}

\subsection{Discussion}
\label{section:discussion}
In this part, we present some discussion of training details and the comparison with RocketQA.

\paratitle{Training Details}
As shown in the Figure~\ref{fig:pipeline}, we organize the above two technical contribution into an effective training pipeline.

\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,labelindent=0cm,leftmargin=0cm]
    \item \textbf{Step 1:} Construct both undenoised instance and denoised instance as hybrid training data by hybrid data augmentation.
    \item \textbf{Step 2:} Perform joint training of the retriever and the re-ranker with dynamic distillation. The warm start models of joint training are RocketQA retriever and re-ranker. In dynamic distillation, the supervised signal of the retriever comes entirely from the re-ranker, since the poor ability of the warm start re-ranker will hinder the learning of retriever at beginning. So that, the joint training needs to start based on two modules that already have certain ability.
\end{itemize}

After completing the training pipeline, we can obtain the optimal retriever and re-ranker for inference.


% In hybrid data augmentation, the existing retriever and re-ranker used for recall and denoising are also implemented based on the two models used for warm start. The first type of data is constructed by the recall results of RocketQA retriever and the second type of data is constructed by both the recall results of RocketQA retriever and denoising results of RocketQA re-ranker. We merge the two types of data for final hybrid training data, and feed to re-ranker for supervision.

% Based on the warm start model and the hybrid training data, we can further implement joint training to obtain two well-trained models. 

\paratitle{Comparison with RocketQA}
Comparing with RocketQA, RocketQAv2 has the following enhancements: 

(1) \emph{A simplified process}. In RocketQAv2, we merge the rest of 3 steps in RocketQA after step 2 into one-step training process\footnote{Since RocketQA mainly focus on retriever training, it totally has 4 training steps without refining the re-ranker. To obtain a better re-ranker, one more step is necessary to train the re-ranker for adapting to the retriever distribution.}, including dual-encoder training with denoised hard negatives, dual-encoder training with data augmentation and cross-encoder training based on dual-encoder. Instead, RocketQAv2 only needs to jointly train the dual-encoder and the cross-encoder with dynamic distillation once to obtain two models with optimal capabilities at the same time. It greatly reduced the cost of iterative training and also achieves a better performance. Moreover, RocketQAv2 only needs 2-3 epochs training to converge, which also decrease the training time cost.

(2) \emph{A more efficient and effective distillation approach}. RocketQA uses hard label for data distillation that the relevance scores of positive instance and negative instance have to be forcibly mapped to 1 and 0, respectively. Hard label for training ignores the intermediate relevance guidance signal and may bring under-learning issue for the retriever. While RocketQAv2 adopts soft relevance score for dynamic distillation, where soft relevance score allows the distillation process to avoid the polarization scoring problem of hard distillation, and dynamic distillation process allows re-ranker to adapt to the relevance distribution of retriever, while allows retriever to touch multi-view of the training data by dynamic updated re-ranker. Both of the two merits make the distillation process more efficient and effective.




%\paratitle{Joint Training}\quad
\ignore{
To achieve joint training, we mainly focus on two aspects: First, we propose dynamic distillation in Section~\ref{section:distill} to enable the information of both retriever and re-ranker to interact with each other during joint training. Besides, the proposed hybrid data augmentation in Section~\ref{section:negative-sampling} incorporates more hard negatives in the joint training process. The large number of hard negatives in the sampling list can better simulate the score distribution of the retriever and the re-ranker, which makes important support to the dynamic distillation.

In joint training architecture, both the retriever and the re-ranker are optimized synchronously. Considering Eq.(\ref{equation:tot_loss}), the retriever tries to approximate the score distribution of the re-ranker by Eq.(\ref{equation:kl_divergence}), the re-ranker learning the supervised data by Eq.(\ref{equation:sup}) and also be optimized according to the score distribution of the retriever by Eq.(\ref{equation:kl_divergence}).
With the merits of our joint training architecture, the retriever and the re-ranker can be directly applied to inference with optimal performance, without the need of iteratively training both models to refer their score distribution to each other.}

%\paratitle{Sampling Strategies}\quad
%In the enhanced multiple negative sampling method, we propose to increase a large number of hard negatives for supporting dynamic soft distillation. Concretely, we adopt two types of sampling strategies for each query $q$. First, we use the labeled passages in dataset as positive passages, the corresponding hard negatives are random sampled in top-$k$ recalled passages from a large passage collection by the existing DPR retriever~\cite{dpr2020}. Besides, Inspired by RocketQA~\citep{rocketqa}, we generate denoised hard negatives for training, where top-retrieved passages that are likely to be false negatives are removed by utilizing a well-trained cross-encoder. Similarly, we also generate corresponding positives through the denoising process by removing top-retrieved passages that are likely to be false positives, this part of positives are not leveraged in RocketQA. Finally, we use one positive passage and $n-1$ hard negatives in the candidate passage list $\mathcal{P}_q$ of the query $q$, where $n$ is the number of passages in candidate list.


\ignore{In this section, we consider the question of why our proposed joint training approach works. Here, we give an illustration for further discussion.

In deep learning datasets, ``multi-view'' structure is a very common phenomenon~\cite{zhu2020towards}. For examples, in vision tasks, a dog can have multiple features to be recognized, by looking at either of the head feature, or the body feature, or even the tail feature. In natural language processing, one kind of semantic can be elaborated through multiple expressions. The multi-view hypothesis can indeed exist even in the intermediate layers of a neural network. Analogously, we can infer that the result distributions of the retriever and the re-ranker also reflect the features of multi-view, which imply the different kinds of hidden knowledge of the data.

Training under the multi-view structure, the model will quickly learn a subset of these feature views based on the randomness in the learning process~\cite{zhu2020towards}. Our retriever and re-ranker are both dynamically updated with the designed objective, thus for each training step, the feature view are different to other steps. Formally, denote $\mathcal{V}$ as the set of feature views, let $M_{de}, M_{ce} \in \mathcal{V}$ be the subset features learned by retriever and re-ranker starting from (independent) random initializations respectively when trained on the original dataset. If we further jointly train the retriever and the re-ranker by dynamic soft distillation for one or few steps, the retriever are going to learn a larger set of feature views $M_{de} \cup M_{ce}$ according to Eq.(\ref{equation:kl_divergence}), and the re-ranker also updates its feature to $M'_{ce}$ according to Eq.(\ref{equation:tot_loss}) that contains different views from the former model. With the increase of the number of steps, a large number of feature views can actually be leveraged. Finally, the model learns a wide range of feature views based on dynamic soft distillation. This process is also similar to an ensemble process, which collecting and combining all the feature views to boost the performance. Experiments in Sec~\ref{section:ablation} also verifies that, if only the static distillation is performed, the performance will decrease compared to dynamic soft distillation.}

